Probabilistic Dual Network Architecture Search on Graphs

We present the first differentiable Network Architecture Search (NAS) for Graph Neural Networks (GNNs). GNNs show promising performance on a wide range of tasks, but require a large amount of architecture engineering. First, graphs are inherently a non-Euclidean and sophisticated data structure, leading to poor adaptivity of GNN architectures across different datasets. Second, a typical graph block contains numerous different components, such as aggregation and attention, generating a large combinatorial search space. To counter these problems, we propose a Probabilistic Dual Network Architecture Search (PDNAS) framework for GNNs. PDNAS not only optimises the operations within a single graph block (micro-architecture), but also considers how these blocks should be connected to each other (macro-architecture). The dual architecture (micro- and marco-architectures) optimisation allows PDNAS to find deeper GNNs on diverse datasets with better performance compared to other graph NAS methods. Moreover, we use a fully gradient-based search approach to update architectural parameters, making it the first differentiable graph NAS method. PDNAS outperforms existing hand-designed GNNs and NAS results, for example, on the PPI dataset, PDNAS beats its best competitors by 1.67 and 0.17 in F1 scores.

==> tables/activation_types.tex <==
\begin{table}[!h]
\caption{Different types of activation functions.}
\label{tab:act_types}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|l}
\toprule
Activation & Equation\\
\midrule
None & $f(x) = x$ \\
Sigmoid & $f(x) = \frac{1}{1+e^{-x}}$\\
Tanh & $ f(x) = tanh(x)$ \\
Softplus & $ f(x) = \frac{1}{\beta} \log (1+e^{\beta x})$\\
ReLU & $f(x) = Max(0,x)$ \\
LeakyReLU & $f(x) = Max(0,x) + \alpha Min(0,x)$ \\
ReLU6 & $f(x) = Min(Max(0,x),6)$ \\
ELU & $f(x) = Max(0,x) + Min(0, \alpha (e^x-1))$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

